A Grassroots Architecture to Supplant Global Digital Platforms by a Global Digital Democracy

We present an architectural alternative to global digital platforms termed grassroots, designed to serve the social, economic, civic, and political needs of local digital communities, as well as their federation. Grassroots platforms may offer local communities an alternative to global digital platforms while operating solely on the smartphones of their members, forsaking any global resources other than the network itself. Such communities may form digital economies without initial capital or external credit, exercise sovereign democratic governance, and federate, ultimately resulting in the grassroots formation of a global digital democracy.

==> stuff.tex <==

\section{Grassroots Applications}\label{section:applications}

\subsection{Grassroots Social Networking}\label{subsection:social-networking}

Offering an  architecture for social networking in which people have agency over  their personal information and social graph is an open challenge. Here\footnote{This paper is a revision and  extension of~\cite{shapiro2023gsn}} we present a grassroots architecture for serverless, permissionless, peer-to-peer social networks termed \textbf{Grassroots Social Networking} that aims to address this challenge. The architecture is geared for people with networked smartphones---roaming (address-changing) computing devices communicating over an unreliable network (e.g., using UDP).  The architecture incorporates (\ia) 
a decentralized social graph, where each person controls, maintains and stores only their local neighborhood in the graph; (\ib) personal feeds, with authors and followers who create and store the feeds; and (\ic) a  grassroots dissemination protocol, in which communication among people occurs only along the edges of their social graph. The architecture realizes these components using the \emph{blocklace} data structure -- a partially-ordered conflict-free counterpart of the  totally-ordered conflict-based blockchain.
We provide two example Grassroots Social Networking protocols---Twitter-like and WhatsApp-like---and address their security (safety, liveness and privacy),  spam/bot/deep-fake resistance, and implementation, demonstrating how server-based social networks could be supplanted by a grassroots architecture. 

The architecture of server-based social networks---whether centralized (Facebook, X), federated~\cite{raman2019challenges}, or blockchain-based~\cite{DSNP}---results in the network operators obtaining and storing a broad range of personal information of their members, including their online behavior, original content, and social graph.
This ability is at the heart of surveillance capitalism~\cite{zuboff2023age}---the business model of all leading social networks---which perfected the commercial exploitation of personal information and original content with little or no remuneration, the provision of biased information in the service of commercial interests,  and the opaque governance of membership and content, also in the service of commercial interests.  In order to mitigate the damage wrecked by surveillance capitalism, governments attempted to legislate the storage and exploitation of personal information, notably the GDPR~\cite{regulation2016GDPR} and DSA~\cite{regulation2022DSA} regulations by the EU.
While this and other regulations have increased the care with which personal information is handled, it also resulted in people consenting a dozen times a day to surrender ownership and control of their personal information to web sites they visit and applications they use. More importantly,
it has not changed the fundamentals of the surveillance-capitalism business model of global social networking platforms.


\GSN offers a grassroots architecture and protocol~\cite{shapiro2023grassroots,shapiro2023grassrootsBA} for serverless, permissionless, peer-to-peer social networks in which people retain ownership and control over their personal information, original digital content, and social graph. \GSN is geared for roaming personal computing devices, namely smartphones, and is guided by three fundamental concepts: 
\begin{enumerate}[leftmargin=*, partopsep=0pt,topsep=0pt,parsep=0pt]
    \item \textbf{Freedom of Digital Assembly}~\cite{mill1859liberty}, the ability of people to assemble freely digitally, not under the control of, and without surrendering personal information to, any third party.
    \item  \textbf{Digital Sovereignty}~\cite{pohle2021digital}, the ability of people to conduct their social, economic, civic, and political lives in the digital realm solely using the networked computing devices they own and operate (e.g., smartphones), free of third-party control, surveillance, manipulation, coercion, or rent seeking.  %Freedom of digital expression and freedom of digital assembly are cornerstones of digital sovereignty.
    \item \textbf{Grassroots Systems}~\cite{shapiro2023grassroots,shapiro2023grassrootsBA}, which are permissionless distributed system that can have multiple oblivious instances (independent of each other and of any global resources)  that can interoperate once interconnected.  \GSN are an example of grassroots systems: Serverless peer-to-peer smartphone-based social networks supporting multiple independently-budding communities that may merge when a member of one community becomes also a member of another. We note that most systems in the digital realm are not grassroots, including centrally-controlled digital platforms (Facebook) and distributed systems designed to have a single global instance (Bitcoin~\cite{bitcoin}, Ethereum~\cite{buterin2014next}) or to employ a single replicated (Blockchain~\cite{bitcoin}), or distributed (IPFS~\cite{benet2014ipfs}, DHT~\cite{rhea2005opendht}) shared global data structure, and distributed pub/sub systems with a global directory~\cite{chockler2007constructing,chockler2007spidercast,buchegger2009peerson}).    
\end{enumerate}

With these concepts we present the architecture of Grassroots Social Networking (GSN) that supports digital freedom of assembly and digital sovereignty
for people with smartphones. We provide two example Grassroots Social Networking protocols: Twitter-like (which is also LinkedIn- and Instagram-like), and WhatsApp-like, demonstrating how centrally-controlled social networks could be supplanted by a serverless, permissionless, peer-to-peer grassroots architecture. 

The \GSN architcture has three components:
\begin{enumerate}[leftmargin=*]
    \item \textbf{Decentralized\footnote{By \emph{decentralized} we mean decentralized control,  so that each agent controls only part of the data structure. Contrast this with standard blockchain applications, where all miners vie for control of the blockchain's single tip.} Social Graph}, with each member controlling, maintaining and storing its local neighbourhood in the graph.  
    \item \textbf{Member-Created Feeds}, each with authors and followers.
    \item \textbf{Grassroots Dissemination}~\cite{shapiro2023grassroots}, a peer-to-peer protocol carried over the edges of the social graph, where friends update each other with information they know and believe their friends need.
\end{enumerate} 

The GSN architecture realizes these components using the \textbf{blocklace} data structure~\cite{shapiro2023grassroots,keidar2022cordial,lewispye2023flash} -- the distributed\footnote{A data structure is \emph{distributed} if different agents access, maintain and store different parts of the data structure.  It is \emph{replicated} if all agents must obtain and maintain a complete copy of the entire data structure in order to operate, as is the norm in blockchain applications.  Note that the term  `distributed ledger' is often used to refer to a replicated ledger.}  partially-ordered counterpart of the replicated totally-ordered blockchain. The blocklace uses blocks to record the evolving social graph; to immutably record acts and their causal relations, supporting members in creating and following feeds; and to function as multichannel ack/nacks, supporting dissemination over an unreliable network.

The Twitter-like network has \emph{public feeds}, each with a sole author and permissionless followers. The WhatsApp-like network has \emph{private groups}, members of each group being both the authors and followers of its feed. Naturally, an actual Grassroots Social Networking application may integrate the two protocols to provide both public feeds and private groups.

   
\GSN is based on two principles:


%\begin{tcolorbox}[colback=gray!5!white,colframe=black!75!black]
\vspace{0.5em}
\fcolorbox{gray!100}{gray!5}{%
    \parbox{0.96\textwidth}{%
        %\lipsum[1]
\textbf{Principles of \GSN:}
\begin{enumerate}[leftmargin=*]
    \item \textbf{Friendship}: Make friends by mutual consent. 
    \item \textbf{Grassroots Dissemination}: Tell to your friends things you know and believe they need.
\end{enumerate}
        }
    }
\vspace{0.5em}
\newline
%\end{tcolorbox}
\GSN realizes these principles using three components:

\vspace{0.5em}
%\begin{tcolorbox}[colback=gray!5!white,colframe=black!75!black]
\fcolorbox{gray!100}{gray!5}{%
    \parbox{0.96\textwidth}{%
    \textbf{Components of \GSN:}
\begin{enumerate}[leftmargin=*]
    \item \textbf{Decentralized Social Graph}, with members controlling, maintaining, and storing their social neighbourhoods in the graph,  e.g., own vertex and adjacent edges.
    \item \textbf{Member-Created Feeds},  with authors and followers.
    \item \textbf{Grassroots Dissemination}, a protocol for communication along the edges of the social graph, through which friends update each other with information they know and believe their friends need.
\end{enumerate}
     }
    }
    \vspace{0.5em}
\newline
%\end{tcolorbox}
All these components are realized via the blocklace, as follows:

\vspace{0.5em}
%\begin{tcolorbox}[colback=gray!5!white,colframe=black!75!black]
\fcolorbox{gray!100}{gray!5}{%
    \parbox{0.96\textwidth}{%
\textbf{In \GSN, the blocklace:}
\begin{enumerate}[leftmargin=*]
    \item \textbf{Social Graph}: Encodes the evolving decentralized social graph, allowing members to create, maintain and store their neighbourhood in the graph.
    \item \textbf{Feeds}:  Immutably records utterances and their causal relations for members to create and follow feeds.
    \item \textbf{Dissemination}: Provides multichannel ack/nacks for grassroots dissemination over an unreliable network.
\end{enumerate}
   }
    }
    

%\end{tcolorbox}
\vspace{0.5em}
We elaborate on each of these components in turn.

\subsection{Grassroots Cryptocurrencies}\label{subsection:cryptocurrencies}


Grassroots currencies are means for turning mutual trust into liquidity, with the goal of providing foundations for grassroots digital economies. Grassroots coins are units of debt that can be issued by anyone---people, corporations, cooperatives, banks, municipalities and governments---and traded by anyone.  They are more similar to `inside money' (a medium of exchange backed by private credit) and to fiat currencies (for which the issuer controls scarcity) than to global cryptocurrencies such as Bitcoin or Ethereum, which are unbacked and for which scarcity is controlled by the protocol.  

Grassroots currencies are mutually-pegged by \emph{coin redemption}: The obligation of a person to redeem any grassroots coin they have issued against any grassroots coin they hold. Coin redemption integrates grassroots currencies issued within a society enjoying a sufficient level of mutual trust into a single liquid economy. 

Grassroots currencies can allow a multitude of local digital economies to emerge without initial capital or external credit, and gradually to merge into a global digital economy.  They are amenable to a simple, serverless, grassroots implementation that requires only interconnected smartphones and is independent of any global digital platforms or other global resources.
As such, grassroots currencies may empower deprived societies worldwide by harnessing mutual trust within the society into internal liquidity and can help `banking the unbanked' along the way.  These abilities may be most relevant in societies in which capital and external credit are scarce but mutual trust due to family, social, and business ties is abundant.

In this paper we introduce the principles that underlie grassroots currencies; 
show that they naturally admit basic fiat currency measures regarding foreign trade such as foreign debt, trade balance, and velocity, and basic accounting measures such as cash ratio, quick ratio, and current ratio; 
elaborate economic scenarios enabled by these principles for grassroots currencies issued by natural and legal persons;
relate grassroots currencies to extant work, including notions of personal currencies, community currencies, cryptocurrencies, and inside money; 
formally specify grassroots currencies as digital entities, governed by the Grassroots Currencies Protocol; discuss the security (safety, liveness, and privacy) of the protocol;
and prove that the protocol is grassroots.  
An implementation of grassroots currencies via a blocklace-based payment system is described elsewhere~\cite{lewis2023grassroots}.



\mypara{Overview} Grassroots currencies are means for turning mutual trust into liquidity.  Their coins are units of debt that can be issued by anyone, natural and legal persons: people, communities, cooperatives, corporations, banks, municipalities and local and federal governments---and traded by anyone.  
Grassroots currencies achieve liquidity through the mutual exchange of grassroots coins by persons that have mutual trust,  and as such are more similar to `inside money'~\cite{lagos2010inside,lagos2017liquidity}---a medium of exchange backed by private credit---than to global cryptocurrencies such as Bitcoin~\cite{bitcoin} or Ethereum~\cite{buterin2014next}. The purpose of grassroots currencies is to provide a foundation for grassroots digital economies. With grassroots currencies,  a multitude of local digital economies can emerge without initial capital or external credit.  Such local digital economies can operate solely on the networked smartphones of their members, independently of any global resources such as global digital platforms or global cryptocurrencies, and gradually merge into a global digital economy.  As such, grassroots currencies may empower economically-deprived communities worldwide, and by harnessing mutual trust within communities help `banking the unbanked'~\cite{agarwal2017banking,dupas2018banking,bruhn2009economic}.  Grassroots currencies may have the greatest impact and utility in places where capital and external credit are scarce but trust within families and communities is abundant.

A grassroots coin in circulation is an outstanding obligation by its issuer to its holder, and
the amount of grassroots coins in circulation in a digital economy is a measure of the trust among its members.  Grassroots currencies are based on the principle that mutually-trusting persons honour their obligations to each other. The main implication of this principle is that it forsakes external capital or credit, allowing communities to leverage mutual trust into a liquid grassroots digital economy; corporations and cooperatives to form without initial capital by establishing credit based on mutual trust with their employees,  customers and suppliers; all levels of government---if liquid---to endow liquidity to their local economies and tame it, as needed; and mutually-trusting persons to trade across national borders.  

Grassroots currencies are endowed with value by their issuer undertaking to redeem them against their offerings:  Goods and services for people and corporations; interest and transaction fees for banks; taxes for cities and states; and fiat currencies for central banks.  Critically, the offerings of each person must also include all the grassroots coins it holds, including coins issued by other persons. Upon request, a person must redeem any coin it has issued against any coin it holds at a 1:1 exchange rate  (Figure \ref{figure:redemption}). 

\begin{wrapfigure}{r}{5cm}
  \begin{center}
   \includegraphics[width=5cm]{Figs/redeem.jpeg}
  \end{center}
  \caption{\textbf{Coin Redemption:}  The red person holds a blue coin and desires the green coin held by the blue person, and thus transfers the blue coin to the blue person and requests to redeem it against the green coin.  The blue person settles the redemption claim by transferring the green coin in return.
  }
\label{figure:redemption}
\end{wrapfigure}
Coin redemption is key for a digital economy based on grassroots currencies to function, as it: (\ia) Makes coins issued by the same person fungible;  (\ib) Resolves doublespending; (\ic) Allows the revocation of credit; (\iiv) Allows chain payments across mutually-liquid currencies; and (\iv) Pegs mutually-liquid grassroots currencies at a 1:1 exchange rate.

Naturally, insolvency, manifest in the inability of a person to redeem coins they have issued, may lead holders of that person's coins to treat them as bad debt and sell them
on the free marked at a discount, effectively devaluating the insolvent person's currency.

In summary, as each person prices their goods and services in terms of their own currency, liquidity arises from persons holding each other's coins, and is correlated with the amount and distribution of coins in circulation.  As grassroots coins are units of debt, the grassroots coins in circulation in an economy reflect the level of trust among the people, organisations and institutions of that economy.


Grassroots currencies naturally support many structures that emerged in the history of economy, such as community\cite{stodder2016macro,dini2019alter,littera2014idea} and corporate currencies\cite{green2011company}, private banking,  credit unions,  Universal Basic Income\cite{howitt2019roadmap}, and Hawala trust-based fund transfer networks\cite{maimbo2003informal}.  Furthermore, any central bank may issue its own grassroots currency to serve as a Central Bank Digital Currency (CBDC), with which it can provide and withdraw liquidity to its local economies at will, with surgical precision and without leakage, as discussed below.   

The responsibility for the economic and computational integrity of a grassroots currency resides with its issuer---natural person, organisation or institution---and as the value of a grassroots currency depends on such integrity, every person is incentivized to maintain it.
The key Byzantine fault against which cryptocurrencies seek defence is equivocation, or doublespending.  No person has an incentive to doublespend their coins, as such doublespending will be exposed promptly, leading to discreditation.  A person would always be better off issuing new coins and handing them over (thus inflating the number of its coins in circulation), instead of doublespending their own coins, as this which would result in the irreparable harm to the person's credibility, a `bank run' on their coins, and annulling the value of their currency. 



